It Takes Two to Tango: Mixup for Deep Metric Learning

Metric learning involves learning a discriminative representation such that embeddings of similar classes are encouraged to be close, while embeddings of dissimilar classes are pushed far apart. State-of-the-art methods focus mostly on sophisticated loss functions or mining strategies. On the one hand, metric learning losses consider two or more examples at a time. On the other hand, modern data augmentation methods for classification consider two or more examples at a time. The combination of the two ideas is under-studied. In this work, we aim to bridge this gap and improve representations using mixup, which is a powerful data augmentation approach interpolating two or more examples and corresponding target labels at a time. This task is challenging because unlike classification, the loss functions used in metric learning are not additive over examples, so the idea of interpolating target labels is not straightforward. To the best of our knowledge, we are the first to investigate mixing both examples and target labels for deep metric learning. We develop a generalized formulation that encompasses existing metric learning loss functions and modify it to accommodate for mixup, introducing Metric Mix, or Metrix. We also introduce a new metric - utilization, to demonstrate that by mixing examples during training, we are exploring areas of the embedding space beyond the training classes, thereby improving representations. To validate the effect of improved representations, we show that mixing inputs, intermediate representations or embeddings along with target labels significantly outperforms state-of-the-art metric learning methods on four benchmark deep metric learning datasets.

==> tex/checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~??.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Abstract and introduction reflect the challenges, contributions and novelty of our paper.}
  \item Did you describe the limitations of your work?
    \answerYes{Limitations are mentioned in \autoref{sec:frame}, \autoref{sec:mixup-set} and \autoref{sec:ablation}}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We are not aware of any negative societal impacts at the time of submission.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Our paper conforms.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Please refer to \autoref{sec:analysis} and supplementary material for details.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Results are given in \autoref{sec:analysis}. Complete proofs are in the supplementary material.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code is included in supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Full training details are given in \autoref{sec:exp} and the supplementary material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We follow existing works like \cite{kim2020proxy}}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{Our method is not computationally expensive and can be reproduced with any GPU resource available.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the creators of all existing assets. Please refer \autoref{sec:exp} and supplementary material.}
  \item Did you mention the license of the assets?
    \answerNo{All the assets used are open-sourced by respective authors.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We do not have any new asset and all assets are open-sourced.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{All data and code are open-sourced.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{It does not.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNo{Not applicable for our work.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{Not applicable for our work.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNo{Not applicable for our work.}
\end{enumerate}

\end{enumerate}

==> tex/notes.tex <==
%notes

% write in supplementary how you generalize for each of the losses mentioned in Table 2
% have a figure explaining pull-push with lambda 
% make a table with Paper | Network | Emb size | ( NOT IN PAPER )


\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lccc|ccc|ccc|ccc} \toprule
	 \multicolumn{4}{c}{CUB200}    & \multicolumn{3}{c}{CARS-196} & \multicolumn{3}{c}{SOP} & \multicolumn{3}{c}{InShop}   \\ \midrule
	  &1 &2 &4   &1 &2 &4  &1 &10 &100  &1 &10 &20      \\
	\toprule
	
	Triplet~\cite{weinberger2009distance}         &60.48  &72.13  &82.11    &74.84  &83.82  &89.98  &- & - &- &- & - &-     \\
	LiftedStructure~\cite{oh2016deep}         &60.16  &72.35  &81.88    &78.15  &86.03  &90.78  &75.51	&88.20	&95.12 &- & - &-     \\
	NPair~\cite{sohn2016improved}             &58.91  &70.66  &79.98    &72.49  &82.23  &88.51  &- & - &-  &- & - &-    \\
	ProxyNCA~\cite{movshovitz2017no}          &62.76  &73.13  &82.17    &78.42  &85.59  &90.76  &- & - &-  &- & - &-    \\ 
	Margin~\cite{sampling_matters}              &63.00  &74.00  &83.59    &79.60  &86.75  &91.49  &- & - &-  &- & - &-   \\
	ArcFace~\cite{deng2019arcface}            &61.33  &71.84  &80.13    &77.78  &85.14  &89.76  &- & - &-  &- & - &-   \\
	\midrule
	Cont.~\cite{hadsell2006dimensionality}              &61.55	 &73.65	    &83.46	  &77.37	&85.54	&89.78	&66.56	&81.77	&90.92   &85.86 &94.49  &95.94  \\
	Cont. $+$ Input ~\cite{zhang2018mixup}       &63.12  &74.54     &83.54   &78.38	   &86.42	  &91.80  &67.62	&82.01	&91.66    &- & - &- \\
	                                             &(\gp{\tb{+1.57}}) &(\gp{\tb{+0.89}}) &	(\gp{\tb{+0.08}})  &(\gp{\tb{+1.01}}) &(\gp{\tb{+0.88}}) &(\gp{\tb{+2.02}}) &- & - &-    &- & - &- \\
	%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------         
	Cont. $+$ Latent ~\cite{}                    &63.96  &75.05   &84.78	    &80.09	   &87.37	  &91.79	&68.11	&82.65	&91.92  &- & - &-   \\
	                                             &(\gp{\tb{+2.41}}) & (\gp{\tb{+1.40}}) &(\gp{\tb{+1.32}}) &(\gp{\tb{+2.72}}) &(\gp{\tb{+1.83}}) &(\gp{\tb{+2.01}}) &- & - &-   &- & - &-  \\
    %-------------------------------------------------------------------------------------------------------------------------------------------------------------------------	                                             
	Cont. $+$ Tensor ~\cite{verma2019manifold}   &\textbf{64.53}  &75.39    &84.28	    &81.47    &88.23     &92.74  &70.69	&83.77	&92.04    &- & - &- \\
	                                             &(\gp{\tb{+2.98}}) &(\gp{\tb{+1.74}}) &(\gp{\tb{+0.82}}) &(\gp{\tb{+4.1}}) &(\gp{\tb{+2.69}}) &(\gp{\tb{+2.96}}) &- & - &-   &- & - &-  \\
    %-------------------------------------------------------------------------------------------------------------------------------------------------------------------------	                 
	\midrule
	MS~\cite{wang2019multi}                &63.88  &75.22  &84.07   &84.12	&90.68	&94.48	&76.20	&88.65	&95.19   &90.15 &97.64 &98.38  \\
	MS $+$ Input~\cite{zhang2018mixup}     &65.72	&77.00	&85.01	&86.04  &91.65	&94.91  &- & - &-   &- & - &-  \\
	                                       &(\gp{\tb{+1.84}}) &(\gp{\tb{+1.78}}) &(\gp{\tb{+0.94}}) &(\gp{\tb{+1.92}}) &(\gp{\tb{+0.97}}) &(\gp{\tb{+0.43}}) &- & - &-  &- & - &-   \\
	%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------
	                                                     
	MS $+$ Latent~\cite{}                  &66.66	          &77.26	         &85.43	            &86.44	           &91.43	          &94.54	&78.57	&90.23	&96.98   &- & - &-  \\
	                                       &(\gp{\tb{+2.78}}) &(\gp{\tb{+2.04}}) &(\gp{\tb{+1.36}}) &(\gp{\tb{+2.32}}) &(\gp{\tb{+0.75}}) &(\gp{\tb{+0.06}}) &- & - &-  &- & - &-   \\
	%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------
	                                                     
	MS $+$ Tensor~\cite{verma2019manifold} &\textbf{66.93}	  &77.31	         &85.31	            &86.78	           &92.03	          &94.98    &78.90	&90.92	&97.01  &- & - &-   \\
	                                       &(\gp{\tb{+3.05}}) &(\gp{\tb{+2.09}}) &(\gp{\tb{+1.24}}) &(\gp{\tb{+2.66}}) &(\gp{\tb{+1.35}}) &(\gp{\tb{+0.50}}) &- & - &-  &- & - &-   \\
    %-------------------------------------------------------------------------------------------------------------------------------------------------------------------------	     
	\midrule
	PA~\cite{kim2020proxy}                     &66.07	&76.60	&85.04	 &84.16	&90.15	&94.08  &79.30	&91.01	&96.20   &89.30 &97.36 &98.19  \\
	PA $+$ Input~\cite{zhang2018mixup}         &67.39	           &77.58	         &85.52     &84.63	&90.48	&93.90     &- & - &-   &- & - &-  \\
	                                                    &(\gp{\tb{+1.32}}) &(\gp{\tb{+0.98}}) &(\gp{\tb{+0.48}}) & & & & & & &- & - &-\\
    %-------------------------------------------------------------------------------------------------------------------------------------------------------------------------	     	                                                    
	PA $+$ Latent~\cite{}                      &67.37	           &77.47	         &86.07	  &84.89	&90.87	&94.15    &79.94	&91.52	&96.68   &- & - &-  \\
	                                                    &(\gp{\tb{+1.30}}) &(\gp{\tb{+0.87}}) &(\gp{\tb{+1.03}}) & & & & & & &- & - &-\\
    %-------------------------------------------------------------------------------------------------------------------------------------------------------------------------	  
	PA $+$ Tensor~\cite{verma2019manifold}     &67.20	          &77.60	          &85.74  &85.00	&90.33	&94.81     &- & - &-  &- & - &-   \\
	                                                    &(\gp{\tb{+1.13}}) &(\gp{\tb{+1.00}}) &(\gp{\tb{+0.70}}) & & & & & & &- & - &-\\
    %-------------------------------------------------------------------------------------------------------------------------------------------------------------------------	  
	 \bottomrule
\end{tabular}
\caption{embedding size 128 with resnet 50}
\label{tab:metric_r50_128}
\end{table}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
